MC-LSTM: Mass-Conserving LSTM

The success of Convolutional Neural Networks (CNNs) in computer vision is mainly driven by their strong inductive bias, which is strong enough to allow CNNs to solve vision-related tasks with random weights, meaning without learning. Similarly, Long Short-Term Memory (LSTM) has a strong inductive bias towards storing information over time. However, many real-world systems are governed by conservation laws, which lead to the redistribution of particular quantities -- e.g. in physical and economical systems. Our novel Mass-Conserving LSTM (MC-LSTM) adheres to these conservation laws by extending the inductive bias of LSTM to model the redistribution of those stored quantities. MC-LSTMs set a new state-of-the-art for neural arithmetic units at learning arithmetic operations, such as addition tasks, which have a strong conservation law, as the sum is constant over time. Further, MC-LSTM is applied to traffic forecasting, modelling a pendulum, and a large benchmark dataset in hydrology, where it sets a new state-of-the-art for predicting peak flows. In the hydrology example, we show that MC-LSTM states correlate with real-world processes and are therefore interpretable.

==> neuralarithmetictable.tex <==
\begin{table}
    \centering
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}[t]{crlcccrlcc}
        \toprule
        \multicolumn{5}{c}{Recurrent arithmetic} & \multicolumn{5}{c}{Static arithmetic} \\
        \midrule
        Op & Method & Success & \multicolumn{2}{c}{Solved at} & Op & Method & Success & \multicolumn{2}{c}{Solved at} \\
        & &  & median & mean &  &  &  & median & mean \\
        \midrule
        
        \multirow{4}{*}{$+$} & \acs{mclstm}\textsubscript{2} & $\mathbf{96\%} {~}^{+2\%}_{-6\%}$ & $4.6 \cdot 10^{5}$ & $4.5 \cdot 10^{5} {~}^{+7.5 \cdot 10^{3}}_{-7.6 \cdot 10^{3}}$ & \multirow{4}{*}{$+$} & \acs{mcfc}\textsubscript{2} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $2.1 \cdot 10^{5}$ & $\mathbf{2.1 \cdot 10^{5}} {~}^{+7.4 \cdot 10^{3}}_{-6.4 \cdot 10^{3}}$  \\
        
        
        & \acs{nau} & $88\% {~}^{+5\%}_{-8\%}$ & $\mathbf{8.1 \cdot 10^{4}}$ & $\mathbf{1.8 \cdot 10^{5}} {~}^{+2.0 \cdot 10^{4}}_{-2.0 \cdot 10^{4}}$ &  & \acs{nau} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $\mathbf{1.8 \cdot 10^{4}}$ & $3.9 \cdot 10^{5} {~}^{+4.5 \cdot 10^{4}}_{-3.7 \cdot 10^{4}}$ \\
        
        & \acs{nalu} &  &  & &  & \acs{nalu} & & & \\
        & \acs{nac} &  &  & &  & \acs{nac} & & & \\

        
        %& & & & & & Gated NAU/NMU & $\mathbf{62\%} {~}^{+9\%}_{-10\%}$ & $\mathbf{1.5 \cdot 10^{6}}$ & $\mathbf{1.5 \cdot 10^{6}} {~}^{+3.9 \cdot 10^{4}}_{-3.8 \cdot 10^{4}}$ \\
        
        \midrule
        %\multirow{3}{*}{$-$} & \acs{mclstm}\textsubscript{3} & $\mathbf{81\%} {~}^{+6\%}_{-9\%}$ & $1.2 \cdot 10^{5}$ & $1.6 \cdot 10^{5} {~}^{+1.5 \cdot 10^{4}}_{-1.4 \cdot 10^{4}}$ & \multirow{3}{*}{$-$}  & \acs{mcfc}\textsubscript{2} & $85\% {~}^{+6\%}_{-8\%}$ & $2.5 \cdot 10^{5}$ & $2.7 \cdot 10^{5} {~}^{+1.7 \cdot 10^{4}}_{-1.7 \cdot 10^{4}}$ \\
        \multirow{4}{*}{$-$} & \acs{mclstm}\textsubscript{3} & $\mathbf{81\%} {~}^{+6\%}_{-9\%}$ & $1.2 \cdot 10^{5}$ & $1.6 \cdot 10^{5} {~}^{+1.5 \cdot 10^{4}}_{-1.4 \cdot 10^{4}}$ & \multirow{4}{*}{$-$}  &  \acs{mcfc}\textsubscript{3} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $1.6 \cdot 10^{5}$ & $1.8 \cdot 10^{5} {~}^{+1.2 \cdot 10^{4}}_{-1.0 \cdot 10^{4}}$ \\
        %& & & & & & \acs{mcfc}\textsubscript{3} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $1.6 \cdot 10^{5}$ & $1.8 \cdot 10^{5} {~}^{+1.2 \cdot 10^{4}}_{-1.0 \cdot 10^{4}}$ \\
    
        & \acs{nau} & $60\% {~}^{+9\%}_{-10\%}$ & $\mathbf{6.1 \cdot 10^{4}}$ & $\mathbf{1.1 \cdot 10^{5}} {~}^{+1.7 \cdot 10^{4}}_{-1.3 \cdot 10^{4}}$ & & \acs{nau} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $\mathbf{5.0 \cdot 10^{3}}$ & $\mathbf{1.6 \cdot 10^{5}} {~}^{+1.7 \cdot 10^{3}}_{-1.6 \cdot 10^{3}}$ \\
        
        & \acs{nalu} &  &  & &  & \acs{nalu} & & & \\
        & \acs{nac} &  &  & &  & \acs{nac} & & & \\

        \midrule
        \multirow{4}{*}{$\cdot$} & \acs{mclstm}\textsubscript{mul} & ? & ? & ? & \multirow{4}{*}{$\cdot$} & \acs{mcfc}\textsubscript{3,mul} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $\mathbf{1.4 \cdot 10^{6}}$ & $\mathbf{1.4 \cdot 10^{6}} {~}^{+1.7 \cdot 10^{4}}_{-1.7 \cdot 10^{4}}$  \\
        
        
        & \acs{nmu} & ? & ? & ? & & \acs{nmu} & $98\% {~}^{+1\%}_{-5\%}$ & $1.4 \cdot 10^{6}$ & $1.5 \cdot 10^{6} {~}^{+5.0 \cdot 10^{4}}_{-6.6 \cdot 10^{4}}$ \\
        & \acs{nalu} &  &  & &  & \acs{nalu} & & & \\
        & \acs{nac} &  &  & &  & \acs{nac} & & & \\

        \bottomrule
    \end{tabular}
    }
    
    \caption{Results for the recurrent arithmetic and static problems.
    "Op" reports the operation that has to be learned in this subtask.
    The column "Method" reports the compared method. The "Success" column reports the percentage of runs that were solved up to
    numeric precision. Error bars represent 95\% confidence intervals.
    The column "Solved at" provides the number of updates required
    to solve the task. \ac{mcfc} is a mass-conserving variant of  \ac{mclstm} 
    based on fully-connected layers for non-recurrent tasks.}
    \label{tab:recurrent}
\end{table}

% \begin{table}
% \parbox{.49\textwidth}{

% \centering
% \begin{tabular}[t]{crllll}
% \toprule
% Op & Model & Success & \multicolumn{2}{c}{Solved at} \\
% \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-5}
%  &  & Rate & Median & Mean \\
% \midrule
% \multirow{2}{*}{$+$} & \acs{mcfc}\textsubscript{2} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $2.1 \cdot 10^{5}$ & $\mathbf{2.1 \cdot 10^{5}} {~}^{+7.4 \cdot 10^{3}}_{-6.4 \cdot 10^{3}}$ \\
% & \acs{nau} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $\mathbf{1.8 \cdot 10^{4}}$ & $3.9 \cdot 10^{5} {~}^{+4.5 \cdot 10^{4}}_{-3.7 \cdot 10^{4}}$ \\
% \midrule
% %\multirow{3}{*}{$-$} & \acs{mcfc}\textsubscript{2} & $85\% {~}^{+6\%}_{-8\%}$ & $2.5 \cdot 10^{5}$ & $2.7 \cdot 10^{5} {~}^{+1.7 \cdot 10^{4}}_{-1.7 \cdot 10^{4}}$ \\
% & \acs{mcfc}\textsubscript{3} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $1.6 \cdot 10^{5}$ & $1.8 \cdot 10^{5} {~}^{+1.2 \cdot 10^{4}}_{-1.0 \cdot 10^{4}}$ \\
% & \acs{nau} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $\mathbf{5.0 \cdot 10^{3}}$ & $\mathbf{1.6 \cdot 10^{5}} {~}^{+1.7 \cdot 10^{3}}_{-1.6 \cdot 10^{3}}$ \\
% \midrule
% \multirow{2}{*}{$\cdot$} & \acs{mcfc}\textsubscript{3,mul} & $\mathbf{100\%} {~}^{+0\%}_{-4\%}$ & $\mathbf{1.4 \cdot 10^{6}}$ & $\mathbf{1.4 \cdot 10^{6}} {~}^{+1.7 \cdot 10^{4}}_{-1.7 \cdot 10^{4}}$ \\
% & \acs{nmu} & $98\% {~}^{+1\%}_{-5\%}$ & $1.4 \cdot 10^{6}$ & $1.5 \cdot 10^{6} {~}^{+5.0 \cdot 10^{4}}_{-6.6 \cdot 10^{4}}$ \\
% \bottomrule
% \end{tabular}
% \caption{Results for the static arithmetic problems. \ac{mcfc}\textsubscript{$N$} corresponds to a \ac{mcfc} layer with $N$ hidden neurons. The \ac{mcfc}\textsubscript{$N$,mul} corresponds to a model with $\exp(\mathrm{\ac{mcfc}}(\log(\alpha x)))$ for the output layer.\label{tab:static}}
% }
% \hfill
% \parbox{.49\textwidth}{
%   \centering
% \begin{tabular}[t]{crllll}
% \toprule
% Op & Model & Success & \multicolumn{2}{c}{Solved at} \\
% \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-5}
%  &  & Rate & Median & Mean \\
% \midrule
% \multirow{2}{*}{$+$} & \acs{mclstm}\textsubscript{2} & $\mathbf{96\%} {~}^{+2\%}_{-6\%}$ & $4.6 \cdot 10^{5}$ & $4.5 \cdot 10^{5} {~}^{+7.5 \cdot 10^{3}}_{-7.6 \cdot 10^{3}}$ \\
% & \acs{nau} & $88\% {~}^{+5\%}_{-8\%}$ & $\mathbf{8.1 \cdot 10^{4}}$ & $\mathbf{1.8 \cdot 10^{5}} {~}^{+2.0 \cdot 10^{4}}_{-2.0 \cdot 10^{4}}$ \\
% \midrule
% \multirow{2}{*}{$-$} & \acs{mclstm}\textsubscript{3} & $\mathbf{81\%} {~}^{+6\%}_{-9\%}$ & $1.2 \cdot 10^{5}$ & $1.6 \cdot 10^{5} {~}^{+1.5 \cdot 10^{4}}_{-1.4 \cdot 10^{4}}$ \\
% & \acs{nau} & $60\% {~}^{+9\%}_{-10\%}$ & $\mathbf{6.1 \cdot 10^{4}}$ & $\mathbf{1.1 \cdot 10^{5}} {~}^{+1.7 \cdot 10^{4}}_{-1.3 \cdot 10^{4}}$ \\
% \midrule
% \multirow{2}{*}{$\cdot$} & \acs{mclstm}\textsubscript{mul} & ? & ? & ? \\
% & \acs{nmu} & ? & ? & ? \\
% \bottomrule
% \end{tabular}

% \caption{Results for the recurrent arithmetic problems. 
% \ac{mcfc}\textsubscript{$N$} corresponds to a \ac{mcfc} 
% layer with $N$ hidden neurons. The \ac{mcfc}\textsubscript{mul} 
% corresponds to $\exp(\mathrm{\ac{mcfc}}(\log(\alpha x)))$. \label{tab:recurrent} }
% }
%   \end{table}

